A Lie bracket approximation approach to distributed optimization over directed graphs

We consider a group of computation units trying to cooperatively solve a distributed optimization problem with shared linear equality and inequality constraints. Assuming that the computation units are communicating over a network whose topology is described by a time-invariant directed graph, by combining saddle-point dynamics with Lie bracket approximation techniques we derive a methodology that allows to design distributed continuous-time optimization algorithms that solve this problem under minimal assumptions on the graph topology as well as on the structure of the constraints. We discuss several extensions as well as special cases in which the proposed procedure becomes particularly simple.

==> myStandardPreamble_arXiv.tex <==
% change @-symbol interpretation for using macros
\makeatletter

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% =============================
% ===         M I S C      ====
% =============================

% extended TeX
\@ifpackageloaded{etex}{}{\RequirePackage{etex}}

% keeps relative paths when including different .tex-files
% use \subimport*{subdirectory}{tex-File} to input tex-Files
\@ifpackageloaded{import}{}{\usepackage{import}}

% nice tables
\@ifpackageloaded{booktabs}{}{\usepackage{booktabs}}

% microtype for better spacing of letters
%\@ifpackageloaded{microtype}{}{\usepackage{microtype}}

% calculations also in tex-Code
\@ifpackageloaded{calc}{}{\usepackage{calc}}

% if conditions
\@ifpackageloaded{ifthen}{}{\usepackage{ifthen}}

% underlining, canceling, ...
\@ifpackageloaded{ulem}{}{\usepackage{ulem}}

% =============================
% ===    G R A P H I C S    ===
% =============================
\@ifpackageloaded{graphicx}{}{\usepackage{graphicx}}
\@ifpackageloaded{xcolor}{}{\usepackage{xcolor}}


% =============================
% ===         T I K Z      ====
% =============================
\@ifpackageloaded{tikz}{
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
     }{
     \usepackage{tikz}
     \usetikzlibrary{arrows,shapes,patterns,positioning,calc}
}
\@ifpackageloaded{pgfplots}{
     }{
     \usepackage{pgfplots}
     }
% SOME TIKZ STYLE DEFINITIONS
\tikzstyle{boxstyle}=[draw=black,inner sep=7pt]      % style for boxes in blockdiagrams
\tikzstyle{arrowstyle}=[]                            % style for arrows in blockdiagrams



% =============================
% ===         M A T H      ====
% =============================
\@ifpackageloaded{amsmath}{}{\usepackage{amsmath}}
\@ifpackageloaded{amsfonts}{}{\usepackage{amsfonts}}
\@ifpackageloaded{amssymb}{}{\usepackage{amssymb}}
\let\theoremstyle\relax
\@ifpackageloaded{amsthm}{}{\usepackage{amsthm}}
\@ifpackageloaded{yhmath}{}{\usepackage{yhmath}}
\@ifpackageloaded{mathdots}{}{\usepackage{mathdots}}


% =============================
% ===    H Y P E R R E F    ===
% =============================

% some color definitions
\colorlet{lcolor}{green!45!black}
\colorlet{ucolor}{magenta!40!black}
\colorlet{ccolor}{green!45!black}

% hyperref for internal links
\usepackage[colorlinks=true,%
            linkcolor=lcolor,%
            urlcolor=lcolor,%
            citecolor=lcolor]{hyperref}

% cleverref for automatically labeling of references
\usepackage[nameinlink]{cleveref}






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% rechange @-symbol interpretation
\makeatother

